Automatic Discrimination of Human and Neural Machine Translation in Multilingual Scenarios

We tackle the task of automatically discriminating between human and machine translations. As opposed to most previous work, we perform experiments in a multilingual setting, considering multiple languages and multilingual pretrained language models. We show that a classifier trained on parallel data with a single source language (in our case German-English) can still perform well on English translations that come from different source languages, even when the machine translations were produced by other systems than the one it was trained on. Additionally, we demonstrate that incorporating the source text in the input of a multilingual classifier improves (i) its accuracy and (ii) its robustness on cross-system evaluation, compared to a monolingual classifier. Furthermore, we find that using training data from multiple source languages (German, Russian, and Chinese) tends to improve the accuracy of both monolingual and multilingual classifiers. Finally, we show that bilingual classifiers and classifiers trained on multiple source languages benefit from being trained on longer text sequences, rather than on sentences.

==> table_versions/blue_orange.tex <==
\begin{tabular}{l|cccccccc|cccccccc}
    \toprule
      & \multicolumn{8}{c|}{\textbf{Trained on Google translations}} & \multicolumn{8}{c}{\textbf{Trained on DeepL translations}} \\
      \midrule
     \textbf{$\downarrow$ Eval} & \textbf{de-d} & \textbf{de-t} & \textbf{fi} & \textbf{gu} & \textbf{kk} & \textbf{lt} & \textbf{ru} & \textbf{zh} & \textbf{de-d} & \textbf{de-t} & \textbf{fi} & \textbf{gu} & \textbf{kk} & \textbf{lt} & \textbf{ru} & \textbf{zh}  \\
     \midrule
    DeepL  & \cellcolor{blue!79.78!orange} \color{white}{ 66.0 } & \cellcolor{blue!60.45!orange} \color{white}{ 57.4 } & \cellcolor{blue!77.08!orange} \color{white}{ 64.8 } &  \centdash  &  \centdash  & \cellcolor{blue!60.9!orange} \color{white}{ 57.6 } & \cellcolor{blue!54.16!orange} \color{white}{ 54.6 } & \cellcolor{blue!52.36!orange} \color{white}{ 53.8 } & \cellcolor{blue!92.58!orange} \color{white}{ 71.7 } & \cellcolor{blue!81.8!orange} \color{white}{ 66.9 } & \cellcolor{blue!85.84!orange} \color{white}{ 68.7  } &  \centdash  &  \centdash  & \cellcolor{blue!85.62!orange} \color{white}{ 68.6 } & \cellcolor{blue!65.17!orange} \color{white}{ 59.5  } & \cellcolor{blue!83.6!orange} \color{white}{  67.7} \\
    Google  & \cellcolor{blue!100.0!orange} \color{white}{ 75.0 } & \cellcolor{blue!78.88!orange} \color{white}{ 65.6 } & \cellcolor{blue!90.56!orange} \color{white}{ 70.8 } & \cellcolor{blue!70.79!orange} \color{white}{ 62.0 } & \cellcolor{blue!85.62!orange} \color{white}{ 68.6 } & \cellcolor{blue!89.44!orange} \color{white}{ 70.3 } & \cellcolor{blue!74.16!orange} \color{white}{ 63.5 } & \cellcolor{blue!62.92!orange} \color{white}{ 58.5  } & \cellcolor{blue!88.76!orange} \color{white}{ 70.0 } & \cellcolor{blue!77.08!orange} \color{white}{   64.8 } & \cellcolor{blue!79.1!orange} \color{white}{ 65.7 } & \cellcolor{blue!65.17!orange} \color{white}{ 59.5 } & \cellcolor{blue!77.75!orange} \color{white}{ 65.1 } & \cellcolor{blue!77.53!orange} \color{white}{ 65.0 } & \cellcolor{blue!67.64!orange} \color{white}{ 60.6 } & \cellcolor{blue!70.34!orange} \color{white}{ 61.8 } \\
    WMT\textsubscript{1}  & \cellcolor{blue!60.22!orange} \color{white}{ 57.3 } & \cellcolor{blue!90.34!orange} \color{white}{ 70.7 } & \cellcolor{blue!82.02!orange} \color{white}{ 67.0 } & \cellcolor{blue!77.98!orange} \color{white}{ 65.2 } & \cellcolor{blue!81.57!orange} \color{white}{ 66.8 } & \cellcolor{blue!72.81!orange} \color{white}{ 62.9 } & \cellcolor{blue!63.6!orange} \color{white}{ 58.8 } & \cellcolor{blue!62.25!orange} \color{white}{ 58.2 } & \cellcolor{blue!68.31!orange} \color{white}{ 60.9  } & \cellcolor{blue!81.57!orange} \color{white}{  66.8 } & \cellcolor{blue!80.9!orange} \color{white}{ 66.5 } & \cellcolor{blue!67.42!orange} \color{white}{ 60.5 } & \cellcolor{blue!75.96!orange} \color{white}{ 64.3 } & \cellcolor{blue!81.8!orange} \color{white}{ 66.9 } & \cellcolor{blue!63.15!orange} \color{white}{ 58.6 } & \cellcolor{blue!79.1!orange} \color{white}{ 65.7 } \\
    WMT\textsubscript{2}  & \cellcolor{blue!62.02!orange} \color{white}{ 58.1 } & \cellcolor{blue!89.21!orange} \color{white}{ 70.2 } & \cellcolor{blue!85.39!orange} \color{white}{ 68.5 } & \cellcolor{blue!73.26!orange} \color{white}{ 63.1 } & \cellcolor{blue!84.72!orange} \color{white}{ 68.2 } & \cellcolor{blue!74.83!orange} \color{white}{ 63.8 } & \cellcolor{blue!59.33!orange} \color{white}{ 56.9 } & \cellcolor{blue!59.78!orange} \color{white}{ 57.1 } & \cellcolor{blue!67.64!orange} \color{white}{ 60.6 } & \cellcolor{blue!79.55!orange} \color{white}{  65.9 } & \cellcolor{blue!76.4!orange} \color{white}{ 64.5 } & \cellcolor{blue!63.82!orange} \color{white}{ 58.9 } & \cellcolor{blue!79.55!orange} \color{white}{ 65.9 } & \cellcolor{blue!84.27!orange} \color{white}{ 68.0 } & \cellcolor{blue!41.8!orange} \color{white}{ 49.1 } & \cellcolor{blue!73.48!orange} \color{white}{ 63.2 } \\
    WMT\textsubscript{3}  & \cellcolor{blue!63.82!orange} \color{white}{ 58.9 } & \cellcolor{blue!77.3!orange} \color{white}{ 64.9 } & \cellcolor{blue!77.98!orange} \color{white}{ 65.2 } & \cellcolor{blue!64.94!orange} \color{white}{ 59.4 } & \cellcolor{blue!90.79!orange} \color{white}{ 70.9 } & \cellcolor{blue!82.02!orange} \color{white}{ 67.0 } & \cellcolor{blue!58.2!orange} \color{white}{ 56.4 } & \cellcolor{blue!52.13!orange} \color{white}{ 53.7 } & \cellcolor{blue!56.63!orange} \color{white}{ 55.7 } & \cellcolor{blue!37.3!orange} \color{white}{  47.1 } & \cellcolor{blue!42.02!orange} \color{white}{ 49.2 } & \cellcolor{blue!18.2!orange} \color{white}{ 38.6 } & \cellcolor{blue!76.4!orange} \color{white}{ 64.5 } & \cellcolor{blue!52.58!orange} \color{white}{ 53.9 } & \cellcolor{blue!35.28!orange} \color{white}{ 46.2 } & \cellcolor{blue!40.45!orange} \color{white}{ 48.5 } \\
    WMT\textsubscript{4}  & \cellcolor{blue!59.55!orange} \color{white}{ 57.0 } & \cellcolor{blue!75.51!orange} \color{white}{ 64.1 } & \cellcolor{blue!38.43!orange} \color{white}{ 47.6 } & \cellcolor{blue!70.34!orange} \color{white}{ 61.8 } & \cellcolor{blue!54.38!orange} \color{white}{ 54.7 } & \cellcolor{blue!69.66!orange} \color{white}{ 61.5 } & \cellcolor{blue!64.94!orange} \color{white}{ 59.4 } & \cellcolor{blue!51.69!orange} \color{white}{ 53.5 } & \cellcolor{blue!37.53!orange} \color{white}{ 47.2 } & \cellcolor{blue!20.9!orange} \color{white}{  39.8 } & \cellcolor{blue!0.0!orange} \color{white}{ 30.5 } & \cellcolor{blue!50.34!orange} \color{white}{ 52.9 } & \cellcolor{blue!25.62!orange} \color{white}{ 41.9 } & \cellcolor{blue!37.08!orange} \color{white}{ 47.0 } & \cellcolor{blue!46.52!orange} \color{white}{ 51.2 } & \cellcolor{blue!55.51!orange} \color{white}{ 55.2 } \\
     \bottomrule
\end{tabular}

==> table_versions/blue_yellow.tex <==
\begin{tabular}{l|cccccccc|cccccccc}
     \toprule
      & \multicolumn{8}{c|}{\textbf{Trained on Google translations}} & \multicolumn{8}{c}{\textbf{Trained on DeepL translations}} \\
      \midrule
     \textbf{$\downarrow$ Eval} & \textbf{de-d} & \textbf{de-t} & \textbf{fi} & \textbf{gu} & \textbf{kk} & \textbf{lt} & \textbf{ru} & \textbf{zh} & \textbf{de-d} & \textbf{de-t} & \textbf{fi} & \textbf{gu} & \textbf{kk} & \textbf{lt} & \textbf{ru} & \textbf{zh}  \\
     \midrule
        DeepL  & \cellcolor{blue!79.78!yellow} \color{white}{ 66.0 } & \cellcolor{blue!60.45!yellow} \color{white}{ 57.4 } & \cellcolor{blue!77.08!yellow} \color{white}{ 64.8 } &  \centdash  &  \centdash  & \cellcolor{blue!60.9!yellow} \color{white}{ 57.6 } & \cellcolor{blue!54.16!yellow} \color{white}{ 54.6 } & \cellcolor{blue!52.36!yellow} \color{white}{ 53.8 } & \cellcolor{blue!92.58!yellow} \color{white}{ 71.7 } & \cellcolor{blue!81.8!yellow} \color{white}{ 66.9 } & \cellcolor{blue!85.84!yellow} \color{white}{ 68.7  } &  \centdash  &  \centdash  & \cellcolor{blue!85.62!yellow} \color{white}{ 68.6 } & \cellcolor{blue!65.17!yellow} \color{white}{ 59.5  } & \cellcolor{blue!83.6!yellow} \color{white}{  67.7} \\
        Google  & \cellcolor{blue!100.0!yellow} \color{white}{ 75.0 } & \cellcolor{blue!78.88!yellow} \color{white}{ 65.6 } & \cellcolor{blue!90.56!yellow} \color{white}{ 70.8 } & \cellcolor{blue!70.79!yellow} \color{white}{ 62.0 } & \cellcolor{blue!85.62!yellow} \color{white}{ 68.6 } & \cellcolor{blue!89.44!yellow} \color{white}{ 70.3 } & \cellcolor{blue!74.16!yellow} \color{white}{ 63.5 } & \cellcolor{blue!62.92!yellow} \color{white}{ 58.5  } & \cellcolor{blue!88.76!yellow} \color{white}{ 70.0 } & \cellcolor{blue!77.08!yellow} \color{white}{   64.8 } & \cellcolor{blue!79.1!yellow} \color{white}{ 65.7 } & \cellcolor{blue!65.17!yellow} \color{white}{ 59.5 } & \cellcolor{blue!77.75!yellow} \color{white}{ 65.1 } & \cellcolor{blue!77.53!yellow} \color{white}{ 65.0 } & \cellcolor{blue!67.64!yellow} \color{white}{ 60.6 } & \cellcolor{blue!70.34!yellow} \color{white}{ 61.8 } \\
        WMT\textsubscript{1}  & \cellcolor{blue!60.22!yellow} \color{white}{ 57.3 } & \cellcolor{blue!90.34!yellow} \color{white}{ 70.7 } & \cellcolor{blue!82.02!yellow} \color{white}{ 67.0 } & \cellcolor{blue!77.98!yellow} \color{white}{ 65.2 } & \cellcolor{blue!81.57!yellow} \color{white}{ 66.8 } & \cellcolor{blue!72.81!yellow} \color{white}{ 62.9 } & \cellcolor{blue!63.6!yellow} \color{white}{ 58.8 } & \cellcolor{blue!62.25!yellow} \color{white}{ 58.2 } & \cellcolor{blue!68.31!yellow} \color{white}{ 60.9  } & \cellcolor{blue!81.57!yellow} \color{white}{  66.8 } & \cellcolor{blue!80.9!yellow} \color{white}{ 66.5 } & \cellcolor{blue!67.42!yellow} \color{white}{ 60.5 } & \cellcolor{blue!75.96!yellow} \color{white}{ 64.3 } & \cellcolor{blue!81.8!yellow} \color{white}{ 66.9 } & \cellcolor{blue!63.15!yellow} \color{white}{ 58.6 } & \cellcolor{blue!79.1!yellow} \color{white}{ 65.7 } \\
        WMT\textsubscript{2}  & \cellcolor{blue!62.02!yellow} \color{white}{ 58.1 } & \cellcolor{blue!89.21!yellow} \color{white}{ 70.2 } & \cellcolor{blue!85.39!yellow} \color{white}{ 68.5 } & \cellcolor{blue!73.26!yellow} \color{white}{ 63.1 } & \cellcolor{blue!84.72!yellow} \color{white}{ 68.2 } & \cellcolor{blue!74.83!yellow} \color{white}{ 63.8 } & \cellcolor{blue!59.33!yellow} \color{white}{ 56.9 } & \cellcolor{blue!59.78!yellow} \color{white}{ 57.1 } & \cellcolor{blue!67.64!yellow} \color{white}{ 60.6 } & \cellcolor{blue!79.55!yellow} \color{white}{  65.9 } & \cellcolor{blue!76.4!yellow} \color{white}{ 64.5 } & \cellcolor{blue!63.82!yellow} \color{white}{ 58.9 } & \cellcolor{blue!79.55!yellow} \color{white}{ 65.9 } & \cellcolor{blue!84.27!yellow} \color{white}{ 68.0 } & \cellcolor{blue!41.8!yellow} \color{white}{ 49.1 } & \cellcolor{blue!73.48!yellow} \color{white}{ 63.2 } \\
        WMT\textsubscript{3}  & \cellcolor{blue!63.82!yellow} \color{white}{ 58.9 } & \cellcolor{blue!77.3!yellow} \color{white}{ 64.9 } & \cellcolor{blue!77.98!yellow} \color{white}{ 65.2 } & \cellcolor{blue!64.94!yellow} \color{white}{ 59.4 } & \cellcolor{blue!90.79!yellow} \color{white}{ 70.9 } & \cellcolor{blue!82.02!yellow} \color{white}{ 67.0 } & \cellcolor{blue!58.2!yellow} \color{white}{ 56.4 } & \cellcolor{blue!52.13!yellow} \color{white}{ 53.7 } & \cellcolor{blue!56.63!yellow} \color{white}{ 55.7 } & \cellcolor{blue!37.3!yellow} \color{white}{  47.1 } & \cellcolor{blue!42.02!yellow} \color{white}{ 49.2 } & \cellcolor{blue!18.2!yellow} \color{white}{ 38.6 } & \cellcolor{blue!76.4!yellow} \color{white}{ 64.5 } & \cellcolor{blue!52.58!yellow} \color{white}{ 53.9 } & \cellcolor{blue!35.28!yellow} \color{white}{ 46.2 } & \cellcolor{blue!40.45!yellow} \color{white}{ 48.5 } \\
        WMT\textsubscript{4}  & \cellcolor{blue!59.55!yellow} \color{white}{ 57.0 } & \cellcolor{blue!75.51!yellow} \color{white}{ 64.1 } & \cellcolor{blue!38.43!yellow} \color{white}{ 47.6 } & \cellcolor{blue!70.34!yellow} \color{white}{ 61.8 } & \cellcolor{blue!54.38!yellow} \color{white}{ 54.7 } & \cellcolor{blue!69.66!yellow} \color{white}{ 61.5 } & \cellcolor{blue!64.94!yellow} \color{white}{ 59.4 } & \cellcolor{blue!51.69!yellow} \color{white}{ 53.5 } & \cellcolor{blue!37.53!yellow} \color{white}{ 47.2 } & \cellcolor{blue!20.9!yellow} \color{white}{  39.8 } & \cellcolor{blue!0.0!yellow} \color{white}{ 30.5 } & \cellcolor{blue!50.34!yellow} \color{white}{ 52.9 } & \cellcolor{blue!25.62!yellow} \color{white}{ 41.9 } & \cellcolor{blue!37.08!yellow} \color{white}{ 47.0 } & \cellcolor{blue!46.52!yellow} \color{white}{ 51.2 } & \cellcolor{blue!55.51!yellow} \color{white}{ 55.2 } \\
        
    \bottomrule
\end{tabular}

==> table_versions/regular.tex <==
\begin{tabular}{l|cccccccc|cccccccc}
     \toprule
      & \multicolumn{8}{c|}{\textbf{Trained on Google translations}} & \multicolumn{8}{c}{\textbf{Trained on DeepL translations}} \\
      \midrule
     \textbf{$\downarrow$ Eval} & \textbf{de-d} & \textbf{de-t} & \textbf{fi} & \textbf{gu} & \textbf{kk} & \textbf{lt} & \textbf{ru} & \textbf{zh} & \textbf{de-d} & \textbf{de-t} & \textbf{fi} & \textbf{gu} & \textbf{kk} & \textbf{lt} & \textbf{ru} & \textbf{zh}  \\
     \midrule
      DeepL & 66.0 &  57.4 & 64.8 & \centdash & \centdash & 57.6 & 54.6 & 53.8 & 71.7 & 66.9 & 68.7  & \centdash & \centdash & 68.6 & 59.5  &  67.7\\
      Google & 75.0 & 65.6 & 70.8 & 62.0 & 68.6 & 70.3 & 63.5 & 58.5  & 70.0 &   64.8 & 65.7 & 59.5 & 65.1 & 65.0 & 60.6 & 61.8 \\
      WMT\textsubscript{1} & 57.3 & 70.7 & 67.0 & 65.2 & 66.8 & 62.9 & 58.8 & 58.2 & 60.9  &  66.8 & 66.5 & 60.5 & 64.3 & 66.9 & 58.6 & 65.7 \\
      WMT\textsubscript{2} & 58.1 & 70.2 & 68.5 & 63.1 & 68.2 & 63.8 & 56.9 & 57.1 & 60.6 &  65.9 & 64.5 & 58.9 & 65.9 & 68.0 & 49.1 & 63.2 \\
      WMT\textsubscript{3} & 58.9 & 64.9 & 65.2 & 59.4 & 70.9 & 67.0 & 56.4 & 53.7 & 55.7 &  47.1 & 49.2 & 38.6 & 64.5 & 53.9 & 46.2 & 48.5 \\
      WMT\textsubscript{4} & 57.0 & 64.1 & 47.6 & 61.8 & 54.7 & 61.5 & 59.4 & 53.5 & 47.2 &  39.8 & 30.5 & 52.9 & 41.9 & 47.0 & 51.2 & 55.2 \\
     \bottomrule
\end{tabular}
